Continual Learning for Instruction Following from Realtime Feedback

We propose and deploy an approach to continually train an instruction-following agent from feedback provided by users during collaborative interactions. During interaction, human users instruct an agent using natural language, and provide realtime binary feedback as they observe the agent following their instructions. We design a contextual bandit learning approach, converting user feedback to immediate reward. We evaluate through thousands of human-agent interactions, demonstrating 15.4% absolute improvement in instruction execution accuracy over time. We also show our approach is robust to several design variations, and that the feedback signal is roughly equivalent to the learning signal of supervised demonstration data.

==> 99-ethics.tex <==
\section{Ethics Statement}

This study received an exemption from the Institutional Review Board of the institution where the research was conducted.
We compensate crowdworkers at an average of \$21.85 USD per hour.
Worker identities are anonymized in the data we release.
The data and models we release are not designed to be directly deployed beyond the \cerealbar scenario. 
In general, deployment of continually learning systems requires guardrails and monitoring to avoid various undesired outcomes, including acquiring behaviors that may harm users. 

==> model.tex <==
\section{Model}
\label{sec:model}
Our policy is implemented as a neural network model taking as input an instruction $\instruction$ of length $n$ and current world state $\state$, and producing a distribution over the action space $\actions$.
First, the instruction $\instruction$ and world state $\state$ are embedded. 
Their embeddings are then combined to produce a distribution over actions using a module adapted from \system{LingUNet}~\cite{Blukis:18visit-predict}.
Section~\ref{sec:sup:model} in the Supplementary Material provides more details about the model implementation and inference.

\paragraph{Input Embeddings}
We embed instructions using a bidirectional recurrent neural network.
The representation of each instruction is a hidden state $\mathbf{h}_n \in \mathbb{R}^m$, where $m$ is the size of the hidden state.
Each world state $\state \in \mathcal{S}$ includes information about the environment and the agent's instruction execution so far.
We use a representation similar to that of \citet{Suhr2019:cerealbar}, with additional features to allow for partial observability.
The environment representation includes information about the terrain, props, cards, and agents in each position. 
Due to partial observability, any information that changes about the world, such as the presence of a card, may be outdated.
The environment representation also includes information about the follower's trajectory so far, the presence of obstacles in the environment, and the follower's observability.
We learn embeddings for each position, resulting in the final environment representation $\mathbf{Q} \in \mathbb{R}^{l \times l \times v}$, where $l$ is the edge size of the environment and $v$ is the embedding size.

After independently embedding the instruction and environment into $\mathbf{h}_n$ and $\mathbf{Q}$, we compute a joint representation by performing text-conditioned $1 \times 1$ convolutions over the environment representation. 
Element-wise concatenation with $\mathbf{Q}$ results in $\mathbf{Q}' \in \mathbb{R}^{l \times l \times (v + f)}$, where $f$ is the number of filters used for the convolution.
$\mathbf{Q}'$ represents the environment using offset coordinates, which do not precisely represent the structure of the hexagonal grid in the \system{CerealBar} environment.
Later stages in the model architecture mix representations of multiple positions, which requires us to accurately represent this hexagonal structure.
We transform the structure of $\mathbf{Q}'$ to axial coordinates~\cite{hoogeboom2018hexaconv}, and translate and rotate the tensor such that the center position represents the agent's current location, and the agent is facing in a consistent direction.
This process results in $\mathbf{A} \in \mathbb{R}^{l^a \times l^a \times (v + f)}$, where $l^a$ is the edge size after the axial transformation.

\paragraph{Action Prediction}
We use \system{LingUNet}~\cite{Blukis:18visit-predict} to map instruction representation $\mathbf{h}_n$ and environment representation $\mathbf{A}$ to a distribution over actions.
We make two major modifications to \citet{Suhr2019:cerealbar}'s implementation.
First, for all convolutions inside \system{LingUNet}, we use hex-based convolutions, where kernels only operate on a subset of each image patch.
Second, we do not perform the final transposed convolution, and instead directly predict a distribution over the action space $\pi(\cdot \mid \instruction, \state; \theta)$ given the output of the final transposed convolutional layer.

\paragraph{Inference}
\label{sec:inference}
We use ensemble-based inference to construct a policy $\pi$ over executable actions $\action \in \actions'$ using voting.
Executing an action in the environment results in a new world state according to the transition function $\transition$, which is nondeterministic from the follower's perspective.
We continue instruction execution until the stop action \texttt{STOP} is sampled, or until the leader manually reboots the follower (Section~\ref{contlearn:sec:training_data}).
The \texttt{STOP} action marks the current instruction as complete, which either results in the follower's turn ending, or it receiving the next instruction to follow.
